Voxel-Based Indoor Reconstruction From HoloLens Triangle Meshes

Current mobile augmented reality devices are often equipped with range sensors. The Microsoft HoloLens for instance is equipped with a Time-Of-Flight (ToF) range camera providing coarse triangle meshes that can be used in custom applications. We suggest to use the triangle meshes for the automatic generation of indoor models that can serve as basis for augmenting their physical counterpart with location-dependent information. In this paper, we present a novel voxel-based approach for automated indoor reconstruction from unstructured three-dimensional geometries like triangle meshes. After an initial voxelization of the input data, rooms are detected in the resulting voxel grid by segmenting connected voxel components of ceiling candidates and extruding them downwards to find floor candidates. Semantic class labels like 'Wall', 'Wall Opening', 'Interior Object' and 'Empty Interior' are then assigned to the room voxels in-between ceiling and floor by a rule-based voxel sweep algorithm. Finally, the geometry of the detected walls and their openings is refined in voxel representation. The proposed approach is not restricted to Manhattan World scenarios and does not rely on room surfaces being planar.

==> figures/workflow.tex <==
% A) Data Preparation
    %   I) Mesh
    %   II) Voxelization & Normal Classification
    % B) Room Detection
    %   III) Ceiling Detection
    %       1) Trace-Through Walls
    %       2) Ceiling Segmentation
    %   IV) Ceiling Refinement
    %       3) Detection of Ceiling Holes
    %       4) Height Interpolation of Ceiling Holes
    %   V) Floor Detection
    %       5) Segmentation of Floor Candidates
    %       6) Identification of Main Floor Segment
    %       7) Height Interpolation
    %   VI) Ceiling & Floor Finalization
    %       8) Ceiling Hole Closing Decision
    %       9) Ceiling & Floor Height Smoothing
    %       10) Wall Initialization 
    % C) Voxel Classification
    %   VII) Voxel Classification Sweep
    % D) Refinement
    %   VIII) Room Surface Completion
    %       11) Room Surface Completion
    %       12) Wall Normal Determination
    %   IX) Wall Geometry Refinement
    %   X) Wall Opening Refinement
    %       13) Wall Opening Refinement
    %       14) Occlusion Test
    %   XI) Result

\pgfdeclarelayer{bg}
\pgfsetlayers{bg,main}

\tikzstyle{preparation} = [rectangle, rounded corners, minimum width=5.2cm,minimum height=0.7cm, text centered, draw=red, fill=red!20]
\tikzstyle{roomdetection} = [rectangle, rounded corners, minimum width=5.2cm,minimum height=0.7cm, text centered, draw=blue, fill=blue!20]
\tikzstyle{voxelclassification} = [rectangle, rounded corners, minimum width=5.2cm,minimum height=0.7cm, text centered, draw=orange, fill=orange!20]
\tikzstyle{refinement} = [rectangle, rounded corners, minimum width=5.2cm,minimum height=0.7cm, text centered, draw=green, fill=green!20]

\tikzstyle{startstop} = [rectangle,inner sep=0pt,text centered,minimum width=5.2cm,minimum height=0.7cm]

\tikzstyle{arraow} = [thick,->,>=stealth]
	
\begin{figure}[h]
\centering
	\begin{tikzpicture}[%
		node distance = 0.3cm,
		every node/.style={font=\sffamily},
		align=center,
		]
		
		\node[startstop] (mesh) {Input mesh\\\includegraphics[width=0.6\columnwidth]{figures/input_mesh_grey.png}};
		
		\node[preparation,below=of mesh] (voxelization) {Voxelization \& Normal Classification\\\includegraphics[width=0.4\columnwidth]{figures/voxelized_normals.png}};
				
		\node[roomdetection,below=of voxelization] (ceilingdetection) {Ceiling Detection\\\includegraphics[width=0.4\columnwidth]{figures/ceiling_detection_upper_floor.png}};
		\node[roomdetection,below=of ceilingdetection] (ceilingrefinement) {Ceiling Refinement};
		\node[roomdetection,below=of ceilingrefinement] (floordetection) {Floor Detection};
		\node[roomdetection, below=of floordetection] (ceilingfloorfinalization) 
		{Ceiling \& Floor Finalization\\\includegraphics[width=0.4\columnwidth]{figures/ceiling_floor_finalized.png}};
		
		\node[voxelclassification, below=of ceilingfloorfinalization] (voxelclassification) 
		{Voxel Classification Sweep\\\includegraphics[width=0.4\columnwidth]{figures/classification_without_refinement.png}};
		
		%\node[refinement,below=of voxelclassification] (roomsurfacecompletion) {Room Surface Completion};
		\node[refinement,below=of voxelclassification] (wallgeomertyrefinement) {Wall Geometry Refinement};
		\node[refinement,below=of wallgeomertyrefinement] (wallopeningrefinement) {Wall Opening Refinement};
		
		\node[startstop, below=of wallopeningrefinement] (result) {\includegraphics[width=0.6\columnwidth]{figures/output_voxel_model.png}\\Result: classified voxel model};
		
		% Trennlinien
		\draw[dashed,draw=lightgray,thick] let \p1=(voxelization),\p2=(ceilingdetection),\p3=(ceilingdetection.north west),\p4=(ceilingdetection.north east) in
			%(\x3-1cm,{(\y1+\y2)/2}) -- (\x4+1cm,{(\y1+\y2)/2});
			(\x3-1cm,-4.9) -- (\x4+1cm,-4.9);
		\draw[dashed,draw=lightgray,thick] let \p1=(ceilingfloorfinalization),\p2=(voxelclassification),\p3=(voxelclassification.north west),\p4=(voxelclassification.north east) in
			%(\x3-1cm,{(\y2-\y1)/2+\y1}) -- (\x4+1cm,{(\y2-\y1)/2+\y1});
			(\x3-1cm,-12.3) -- (\x4+1cm,-12.3);
		\draw[dashed,draw=lightgray,thick] let \p1=(voxelclassification),\p2=(wallgeomertyrefinement),\p3=(wallgeomertyrefinement.north west),\p4=(wallgeomertyrefinement.north east) in
			%(\x3-1cm,{(\y2-\y1)/2+\y1}) -- (\x4+1cm,{(\y2-\y1)/2+\y1});
			(\x3-1cm,-15.35) -- (\x4+1cm,-15.35);
		
		% Verbindungen
		\begin{pgfonlayer}{bg} 
			\draw[thick,->] (0,0) -- (result.north);
		\end{pgfonlayer}
		
		% Seitentext
		\node[rotate=90,scale=1.2,text=blue] at (-3.2,-8.5) {Room Detection};
		\node[rotate=90,scale=1.2,text=green!50!black] at (-3.2,-16.52) {Refinement};
			
	\end{tikzpicture}
	\caption{Processing workflow from input mesh to final classified voxel model.}
	\label{fig:workflow}
\end{figure}
